HELP: The Herschel Extragalactic Legacy Project

We present the Herschel Extragalactic Legacy Project (HELP). This project collates, curates, homogenises, and creates derived data products for most of the premium multi-wavelength extragalactic data sets. The sky boundaries for the first data release cover 1270 deg2 defined by the Herschel SPIRE extragalactic survey fields; notably the Herschel Multi-tiered Extragalactic Survey (HerMES) and the Herschel Atlas survey (H-ATLAS). Here, we describe the motivation and principal elements in the design of the project. Guiding principles are transparent or "open" methodologies with care for reproducibility and identification of provenance. A key element of the design focuses around the homogenisation of calibration, meta data and the provision of information required to define the selection of the data for statistical analysis. We apply probabilistic methods that extract information directly from the images at long wavelengths, exploiting the prior information available at shorter wavelengths and providing full posterior distributions rather than maximum likelihood estimates and associated uncertainties as in traditional catalogues. With this project definition paper we provide full access to the first data release of HELP; Data Release 1 (DR1), including a monolithic map of the largest SPIRE extragalactic field at 385 deg2 and 18 million measurements of PACS and SPIRE fluxes. We also provide tools to access and analyse the full HELP database. This new data set includes far-infrared photometry, photometric redshifts, and derived physical properties estimated from modelling the spectral energy distributions.

==> HELP_Fields_v4_kband.tex <==
\begin{tabular}{|l|r|r|l|r|r|r|r|l|}
\hline
  \multicolumn{1}{|c|}{Name} &
  \multicolumn{1}{c|}{RA} &
  \multicolumn{1}{c|}{Dec} &
  \multicolumn{1}{c|}{Key Data} &
  \multicolumn{1}{c|}{$K_{\rm AB}>23.7$} &
  \multicolumn{1}{c|}{$K_{\rm AB}>22$} &
  \multicolumn{1}{c|}{$K_{\rm AB}>20.75$} &
  \multicolumn{1}{c|}{$K_{\rm AB}>19.5$} &
  \\
\hline
  SSDF & -8.1 & -55.114 & VISTA-VHS &  & 9.7 & 45.0 & 105.0 & \\
  HATLAS-SGP & 1.5 & -32.734 & VISTA-VHS &  & 7.3 & 292.0 & 294.0 & \\
  ELAIS-S1 & 8.8 & -43.585 & VISTA-VIDEO & 2.8 & 2.8 & 3.4 & 8.9 & \\
  Herschel-Stripe-82 & 14.3 & -0.034 & VISTA-VHS &  & 7.5 & 86.2 & 374.0 & \\
  XMM-LSS & 35.1 & -4.528 & VISTA-VIDEO & 1.0 & 10.5 & 13.2 & 21.5 & \\
  CDFS-SWIRE & 53.1 & -28.235 & VISTA-VIDEO & 2.6 & 4.6 & 8.7 & 12.0 & \\
  AKARI-SEP & 70.8 & -53.862 & VISTA-VHS &  &  & 1.7 & 7.3 & \\
  GAMA-09 & 134.7 & 0.513 & VISTA-VIKING &  & 0.4 & 56.2 & 61.2 & \\
  COSMOS & 150.1 & 2.218 & VISTA-ULTRAVISTA & 1.0 & 1.0 & 1.2 & 5.0 & \\
  Lockman-SWIRE & 161.2 & 58.058 & UKIDS-DXS &  & 10.4 & 10.5 & 10.8 & \\
  GAMA-12 & 179.8 & -0.482 & VISTA-VIKING &  & 3.1 & 59.0 & 61.9 & \\
  HDF-N & 189.2 & 62.241 & Various &  &  &  &  & \\
  SA13 & 198.0 & 42.715 & ? & 0.2 & 0.2 & 0.2 & 0.2 & \\
  HATLAS-NGP & 199.5 & 29.215 & UKIDS-LAS &  & 18.1 & 62.1 & 179.0 & \\
  XMM-13hr & 203.6 & 37.918 & ? &  & 0.7 & 0.7 & 0.7 & \\
  EGS & 215.0 & 52.72 & ? &  & 0.1 & 0.7 & 0.7 & \\
  GAMA-15 & 217.6 & 0.456 & VISTA-VIKING &  & 1.2 & 60.2 & 60.9 & \\
  Bo\"otes & 218.1 & 34.173 &  &  & 4.9 & 5.2 & 5.2 & \\
  ELAIS-N1 & 242.9 & 55.071 & UKIDS-DXS &  & 9.4 & 9.8 & 9.9 & \\
  ELAIS-N2 & 249.2 & 41.058 & UKIDS-LAS &  & 0.1 & 0.2 & 0.8 & \\
  xFLS & 259.0 & 59.384 & UKIDS-LAS &  & 0.1 & 2.6 & 2.7 & \\
  SPIRE-NEP & 265.0 & 69.004 & UKIDS-LAS &  &  &  &  & \\
  AKARI-NEP & 270.0 & 66.556 & UKIDS-LAS &  &  &  &  & \\
  Total	&	&	&	& 7.6	&92.1	&718.8	&1221.7\\
\hline\end{tabular}


==> multiwavelength_surveys.tex <==
\section[Multi-wavelength Survey Audit\\{\color{red}Obsolete?}]{Multi-wavelength Survey Audit}\label{appendix:surveys}

In this section we briefly summarise the data that is anticipated to be included
in HELP.   The summaries are grouped into broad wavelength regions over which
the properties are similar.

\begin{table*}
\begin{tabular}{| ll | l | r| r |l| l|}\hline

\multicolumn{2}{|l|}{Wavelength and bands} & Survey & Area & Overlap & DR1 & Reference\\
\multicolumn{2}{|l|}{} &  & [deg.$^2$] & [deg.$^2$] & & \\ \hline

X-ray     & 1kev & XCS & 500 & 10 & No & Romer et al. 2017 \\
UV     &  \\
Optical\\
NIR &    & 2MASS \\
 &    & UKIDSS \\
 &    & VISTA \\
FIR & & IRAS \\
 & & AKARI \\
 & & ISO \\
 & & SWIRE \\
Sub-mm & \\
Radio & \\ \hline 
\end{tabular}
\caption{Summary of significant photometric surveys with public data that overlap with HELP.  
We tabulate: the primary wavelengths of the survey; the survey name; the approximate approximate sky area; the area of overlap with HELP; whether or not the data is included in the HELP DR1; and the primary reference.}

\end{table*}

